NeRF-LOAM: Neural Implicit Representation for Large-Scale Incremental LiDAR Odometry and Mapping

Simultaneously odometry and mapping using LiDAR data is an important task for mobile systems to achieve full autonomy in large-scale environments. However, most existing LiDAR-based methods prioritize tracking quality over reconstruction quality. Although the recently developed neural radiance fields (NeRF) have shown promising advances in implicit reconstruction for indoor environments, the problem of simultaneous odometry and mapping for large-scale scenarios using incremental LiDAR data remains unexplored. To bridge this gap, in this paper, we propose a novel NeRF-based LiDAR odometry and mapping approach, NeRF-LOAM, consisting of three modules neural odometry, neural mapping, and mesh reconstruction. All these modules utilize our proposed neural signed distance function, which separates LiDAR points into ground and non-ground points to reduce Z-axis drift, optimizes odometry and voxel embeddings concurrently, and in the end generates dense smooth mesh maps of the environment. Moreover, this joint optimization allows our NeRF-LOAM to be pre-trained free and exhibit strong generalization abilities when applied to different environments. Extensive evaluations on three publicly available datasets demonstrate that our approach achieves state-of-the-art odometry and mapping performance, as well as a strong generalization in large-scale environments utilizing LiDAR data. Furthermore, we perform multiple ablation studies to validate the effectiveness of our network design. The implementation of our approach will be made available at https://github.com/JunyuanDeng/NeRF-LOAM.

==> stachnisslab-latex.tex <==
%% Standard latex definitions used at the Stachniss-Lab

\usepackage{graphics}           
\usepackage{times}              
\usepackage{amsmath}            
\usepackage{amssymb}            
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{booktabs}
\usepackage{color}
\definecolor{instructioncolor}{rgb}{.5,.5,.5}

\newcommand{\instruction}[1]{\textcolor{instructioncolor}{#1}}

% make caption font small for better separation of figures and text
\usepackage[font=small]{caption}

 %% Key definitions for text elements. USE ONLY THEM! Do not use naked \ref{}.
\def\secref#1{Sec.~\ref{#1}}
\def\figref#1{Fig.~\ref{#1}}
\def\tabref#1{Tab.~\ref{#1}}
\def\eqref#1{Eq.~(\ref{#1})}
\def\algref#1{Alg.~\ref{#1}}

%% Other useful macros
\newcommand\todo[1]{\textbf{[TODO: #1}]}

\makeatletter
\usepackage{xspace}
%% the \onedot macro is producing only one dot at line ends.
%% thus \etal. will not produce et al..
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{e.g\onedot} \def\Eg{E.g\onedot}
\def\ie{i.e\onedot} \def\Ie{I.e\onedot}
\def\cf{cf\onedot} \def\Cf{Cf\onedot}
\def\etc{etc\onedot} \def\vs{vs\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
%% Cyrill does not like emph...
%\def\etal{\emph{et al}\onedot}
\def\etal{{et al}\onedot}
\makeatother

\def\etalcite#1{\etal~\cite{#1}}

\usepackage{array}
%% this allows to use something like p{2cm} as column type, but with left, center, and right alignment
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}




==> stachnisslab-math.tex <==
%% Math definitions used at the Stachniss-Lab

% argmax operator
\def\argmax{\mathop{\rm argmax}}

% argmain operator
\def\argmin{\mathop{\rm argmin}}

%% Spaces
\newcommand{\PP}{\mathbb{P}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\ZZ}{\mathbb{Z}}

% O-Notation
\newcommand{\bigO}[1]{$\mathcal{O}(#1)$}

% absolute value
\newcommand{\abs}[1]{|#1|}

% Norm
\newcommand{\norm}[1]{\lVert#1\lVert}

% 1/2 as math
\newcommand{\half}{\frac{1}{2}}

% sign 
\newcommand{\sign}[0]{{\mbox{sign}}}

% specif matrix dimensions under a matrix
\newcommand{\mdim}[3]{\stackrel[\mbox{\tiny $#2\!\!\times\!\!#3$}]{}{#1}}

% math boldface #1  
\renewcommand{\b}[1]{\mbox{\boldmath$#1$}}

% =\b (for compatability)
\renewcommand{\d}[1]{\b {#1}}

% vector
\renewcommand{\v}[1]{{\b #1}} 

% matrix
\newcommand{\m}[1]{{\mbox{{\sffamily\slshape{#1\/}}}}}

% homogeneous vector
\newcommand{\q}[1]{{{\bf #1}}}

% homogeneous matrix
\newcommand{\mq}[1]{{\mbox{{\sffamily{#1}}}}}

% transpose vector or matrix
\newcommand{\tr}[0]{\sf T}              % transpose without ^  
\newcommand{\trans}[0]{^\tr}            % normal
\newcommand{\transs}[0]{{'}^\tr}        % ‘ trans
\newcommand{\transss}[0]{{''}^\tr}      % ‘‘ trans
\newcommand{\transsss}[0]{{'''}^\tr}    % ’’’ trans
\newcommand{\transi}[0]{^{-\tr}}        % - trans
\newcommand{\transa}[0]{^{*\tr}}        % * trans

%inverse 
\newcommand{\inv}{^{-1}}

% Differential operator d
\newcommand{\diff}[0]{\mbox{d}}

% degree
\newcommand{\degrees}{{\mbox{$^\circ$}}}

% Diag 
\newcommand{\Diag}[0]{{\mbox{Diag}}}

% trace  
\newcommand{\trace}[0]{{\mbox{tr}\,}}

% rank 
\newcommand{\rank}[0]{{\mbox{rank}\,}}

% nullspace 
\newcommand{\nullspace}[0]{{\mbox{null}}}

%atan2 (use with one argument: sin- and cos-part  seperated by , or ;)
\newcommand{\atan}[1]{\mbox{atan2} \, ({#1})}

%acot2 (use with one argument: sin- and cos-part  seperated by , or ;)
\newcommand{\acot}[1]{\mbox{acot2} \, ({#1})}

% specify coordinate system of an element
%#1 = system, #2 = variable
\newcommand{\cs}[2]{\; ^{#1}\!\,{\mbox{#2}}}

% specify coordinate system of matrix from to
% #1 = variable, #2 = from, #3 = to,
\newcommand{\cft}[3]{\; ^{#1}\!\,{\mbox{#2}}_{#3}}

%Rotationmatrix with index and angle: R_i(a)%
\newcommand{\rot}[2]{\m{R}_{#1}(#2)}

%Rotationmatrix transposed with index and angle:  R^T_i(a)%
\newcommand{\rott}[2]{\m{R}\trans_{#1}(#2)}

% Jacobian
\newcommand{\J}{\m J} 


%2 vector%
\newcommand{\zvector}[2]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2}
        \end{array}
       \right] }

%3 vector%
\newcommand{\dvector}[3]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3}
        \end{array}
       \right] }

%4 vector%
\newcommand{\vvector}[4]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}
          \end{array}
       \right] }

%5 vector%
\newcommand{\fvector}[5]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}
          \end{array}
       \right] }

%%6 vector%
\newcommand{\svector}[6]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}\\ {#6}
          \end{array}
       \right] }

%%7 vector%
\newcommand{\sivector}[7]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}\\ {#6}\\ {#7}
          \end{array}
       \right] }

%%8 vector%
\newcommand{\avector}[8]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}\\ {#6}\\ {#7}\\ {#8}
          \end{array}
       \right] }
       
%%9 vector%
\newcommand{\nvector}[9]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}\\ {#6}\\ {#7}\\ {#8}\\ {#9}
          \end{array}
       \right] }


%2 vector transposed%
\newcommand{\zvectort}[2]
  {    \left[
            {#1} \; {#2}
       \right] }


%3 vector transposed%
\newcommand{\dvectort}[3]
  {    \left[
            {#1} \; {#2}\; {#3}
       \right] }

%4 vector transposed%
\newcommand{\vvectort}[4]
  {    \left[
            {#1} \; {#2}\; {#3}\; {#4}
       \right] }


%2 x 3 matrix%
\newcommand{\zdmatrix}[6]
  {    \left[
          \begin{array}{ccc}
            {#1} & {#2} & {#3} \\
            {#4} & {#5} & {#6} 
          \end{array}
       \right] }

%2 x 4 matrix%
\newcommand{\zvmatrix}[8]
  {    \left[
          \begin{array}{cccc}
            {#1} & {#2} & {#3} & {#4}\\
            {#5} & {#6} & {#7} & {#8}
          \end{array}
       \right] }
%4 x 2 matrix%
\newcommand{\vzmatrix}[8]
  {    \left[
          \begin{array}{cc}
            {#1} & {#2} \\ {#3} & {#4}\\
            {#5} & {#6} \\ {#7} & {#8}
          \end{array}
       \right] }

%3 x 2 matrix%
\newcommand{\dzmatrix}[6]
  {    \left[
          \begin{array}{ccc}
            {#1} & {#2} \\
            {#3} & {#4} \\
            {#5} & {#6}
          \end{array}
       \right] }
%

%2 x 2 matrix%
\newcommand{\zmatrix}[4]
  {    \left[
          \begin{array}{cc}
            {#1} & {#2} \\
            {#3} & {#4}
          \end{array}
       \right] }

%3 x 3 matrix%
\newcommand{\dmatrix}[9]
  {    \left[
          \begin{array}{ccc}
            {#1} & {#2} & {#3} \\
            {#4} & {#5} & {#6} \\
            {#7} & {#8} & {#9}
          \end{array}
       \right] }

%4 x 4 matrix%
%% not allowed, max 9 parameters!

%Determinant 2x2
\newcommand{\zdet}[4]
  {    \left|
          \begin{array}{cc}
            {#1} & {#2} \\
            {#3} & {#4}
          \end{array}
       \right| }

%Determinant 3x3
\newcommand{\ddet}[9]
  {    \left|
          \begin{array}{ccc}
            {#1} & {#2} & {#3}\\
            {#4} & {#5} & {#6}\\
            {#7} & {#8} & {#9}
          \end{array}
       \right| }


 
% General matrix: #1: #colums, #2: String for elemets
% incl. //
\newcommand{\matr}[2]{%
\left[ \begin{array}{*#1{c} }    #2   \end{array} \right] %
  }

 % General Determinant:  #1: #colums, #2: String for elemets
% incl. //
\newcommand{\dete}[2]{%
\left| \begin{array}{*#1{c}}    #2   \end{array} \right| %
  }

 % Boldface abbrevs
\newcommand{\bA}{\b A}
\newcommand{\bB}{\b B}
\newcommand{\bC}{\b C}
\newcommand{\bD}{\b D}
\newcommand{\bE}{\b E}
\newcommand{\bF}{\b F}
\newcommand{\bG}{\b G}
\newcommand{\bH}{\b H}
\newcommand{\bI}{\b I}
\newcommand{\bJ}{\b J}
\newcommand{\bK}{\b K}
\newcommand{\bL}{\b L}
\newcommand{\bM}{\b M}
\newcommand{\bN}{\b N}
\newcommand{\bO}{\b O}
\newcommand{\bP}{\b P}
\newcommand{\bQ}{\b Q}
\newcommand{\bR}{\b R}
\newcommand{\bS}{\b S}
\newcommand{\bT}{\b T}
\newcommand{\bU}{\b U}
\newcommand{\bV}{\b V}
\newcommand{\bW}{\b W}
\newcommand{\bX}{\b X}
\newcommand{\bY}{\b Y}
\newcommand{\bZ}{\b Z}

\newcommand{\ba}{\b a}
\newcommand{\bb}{\b b}
\newcommand{\bc}{\b c}
\newcommand{\bd}{\b d}
\newcommand{\be}{\b e}
%\newcommand{\bf}{\b f}
\newcommand{\bg}{\b g}
\newcommand{\bh}{\b h}
\newcommand{\bi}{\b i}
\newcommand{\bj}{\b j}
\newcommand{\bk}{\b k}
\newcommand{\bl}{\b l}
\newcommand{\bm}{\b m}
\newcommand{\bn}{\b n}
\newcommand{\bo}{\b o}
\newcommand{\bp}{\b p}
\newcommand{\bq}{\b q}
\newcommand{\br}{\b r}
\newcommand{\bs}{\b s}
\newcommand{\bt}{\b t}
\newcommand{\bu}{\b u}
\newcommand{\bv}{\b v}
\newcommand{\bw}{\b w}
\newcommand{\bx}{\b x}
\newcommand{\by}{\b y}
\newcommand{\bz}{\b z}

\newcommand{\dA}{\b A}
\newcommand{\dB}{\b B}
\newcommand{\dC}{\b C}
\newcommand{\dD}{\b D}
\newcommand{\dF}{\b F}
\newcommand{\dG}{\b G}
\newcommand{\dH}{\b H}
\newcommand{\dI}{\b I}
\newcommand{\dJ}{\b J}
\newcommand{\dK}{\b K}
\newcommand{\dL}{\b L}
\newcommand{\dM}{\b M}
\newcommand{\dN}{\b N}
\newcommand{\dO}{\b O}
\newcommand{\dP}{\b P}
\newcommand{\dQ}{\b Q}
\newcommand{\dR}{\b R}
\newcommand{\dS}{\b S}
\newcommand{\dT}{\b T}
\newcommand{\dU}{\b U}
\newcommand{\dV}{\b V}
\newcommand{\dW}{\b W}
\newcommand{\dX}{\b X}
\newcommand{\dY}{\b Y}
\newcommand{\dZ}{\b Z}

\newcommand{\mA}{\m A}
\newcommand{\mB}{\m B}
\newcommand{\mC}{\m C}
\newcommand{\mD}{\m D}
\newcommand{\mF}{\m F}
\newcommand{\mG}{\m G}
\newcommand{\mH}{\m L}
\newcommand{\mI}{\m I}
\newcommand{\mJ}{\m J}
\newcommand{\mK}{\m K}
\newcommand{\mL}{\m L}
\newcommand{\mM}{\m M}
\newcommand{\mN}{\m N}
\newcommand{\mO}{\m O}
\newcommand{\mP}{\m P}
\newcommand{\mQ}{\m Q}
\newcommand{\mR}{\m R}
\newcommand{\mS}{\m S}
\newcommand{\mT}{\m T}
\newcommand{\mU}{\m U}
\newcommand{\mV}{\m V}
\newcommand{\mW}{\m W}
\newcommand{\mX}{\m X}
\newcommand{\mY}{\m Y}
\newcommand{\mZ}{\m Z}


